VASparse: Towards Efficient Visual Hallucination Mitigation via Visual-Aware Token Sparsification

Large Vision-Language Models (LVLMs) may produce outputs that are unfaithful to reality, also known as visual hallucinations (VH), which significantly impedes their real-world usage. To alleviate VH, various decoding strategies have been proposed to enhance visual information. However, many of these methods may require secondary decoding and rollback, which significantly reduces inference speed. In this work, we propose an efficient plug-and-play decoding algorithm via Visual-Aware Sparsification (VASparse) from the perspective of token sparsity for mitigating VH. VASparse is inspired by empirical observations: (1) the sparse activation of attention in LVLMs, and (2) visual-agnostic tokens sparsification exacerbates VH. Based on these insights, we propose a novel token sparsification strategy that balances efficiency and trustworthiness. Specifically, VASparse implements a visual-aware token selection strategy during decoding to reduce redundant tokens while preserving visual context effectively. Additionally, we innovatively introduce a sparse-based visual contrastive decoding method to recalibrate the distribution of hallucinated outputs without the time overhead associated with secondary decoding. Subsequently, VASparse recalibrates attention scores to penalize attention sinking of LVLMs towards text tokens. Extensive experiments across four popular benchmarks confirm the effectiveness of VASparse in mitigating VH across different LVLM families without requiring additional training or post-processing. Impressively, VASparse achieves state-of-the-art performance for mitigating VH while maintaining competitive decoding speed. Code is available at https://github.com/mengchuang123/VASparse-github.

==> sec/2_observe.tex <==
\section{Empirical Observation}
\label{sec:obs}

In this section, we present the motivation behind our vision-aware token sparsification strategy. We first provide evidence of attention sparsity in LVLMs and observe that vision-agnostic (do not adjust token selection during decoding) sparsification methods can intensify VH. Additionally, we emphasize the necessity of attending to image tokens and applying attention penalties to text tokens prone to attention sinking.


\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{sec/Figure/Obs/VCSparse-2.pdf}
    \caption{Attention between Tokens is Highly Sparse.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{sec/Figure/Obs/VCSparse-1.pdf}
    \caption{Visual-Agnostic Token Sparsification and VH.}
    \label{fig:short-b}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{sec/Figure/Obs/VCSparse-3.pdf}
    \caption{Attention Density of Visual and Textual Tokens.}
    \label{fig:short-c}
  \end{subfigure}
  \caption{Visual hallucination evaluation and attention score analysis using LLaVA-1.5 on the CHAIR benchmark: (a) token sorting by attention score, (b) token sparsification effects observed with Vanilla Top-K, FastV, and SparseVLM on 500 sampled images from the MSCOCO validation set, and (c) attention density distribution across visual and textual tokens.}
  \label{fig:short}
\end{figure*}



\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.85\linewidth]{sec/Figure/Obs/Attn-Sink.pdf}

   \caption{Attention sinking phenomenon in LVLMs: In the 8th Transformer layer of LLaVA-1.5, 26th attention head exhibits a substantial concentration of attention scores on specific text tokens, including tokens \texttt{<.>} and \texttt{<s>}.}
   \label{fig:onecol}
\end{figure}

\subsection{Sparse Activation in LVLM Attention}
\label{subsec:obs-1}
\textbf{Observation}:~
We conduct experiments using LLAVA-1.5 and sort the attention scores calculated for decoded tokens in ascending order. As shown in Figure~\ref{fig:short-a}, we observe a clear long-tail distribution in the attention scores, where only a small subset of tokens is heavily activated during decoding. This indicates that self-attention in the majority of layers in the LVLM decoder is sparse. Retaining only the top 1\% of tokens by attention score can recall over 98\% of the total attention scores.

\textbf{Insights}:~
Our findings substantiate that self-attention in most layers of the LVLM decoder is sparse. This insight suggests the potential for pruning corresponding tokens to reduce computational cost during decoding.

\subsection{Vision-Agnostic Sparsification Aggravates VH}
\label{subsec:obs-2}
\textbf{Observation}:~
We evaluate visual hallucination in the model using LLaVA-1.5 with vision-agnostic token sparsification on a randomly sampled set of 500 images, including the vanilla Top-K strategy, FastV and SparseVLM. As shown in Figure~\ref{fig:short-b}, we observe that as the sparsification level increases, the model becomes more prone to visual hallucination. 

\textbf{Insights}:~
Our empirical findings indicate that these vision-agnostic sparsification techniques exacerbate visual hallucination in the model. This suggests that simply adopting such sparsification methods to accelerate decoding may compromise the fidelity of the model’s output.

\subsection{Distinct Distribution of Image and Text Tokens} 
\label{subsec:obs-3}
\textbf{Observation}:~
We conduct experiments on the CHAIR benchmark using LLAVA-1.5 across 500 randomly sampled images. We analyze the attention distribution of image and text tokens, with results shown in Figure~\ref{fig:short-c}. A clear divergence in distribution is evident: image tokens predominantly occupy lower-attention regions, whereas text tokens concentrate in higher-attention regions.

\textbf{Insights}:~
These findings suggest that LVLMs tend to overlook image tokens during decoding, instead focusing predominantly on text tokens. This observation also explains why vision-agnostic token sparsification strategies may exacerbate hallucinations: they are more likely to prune low-attention image tokens which contain important visual information. This insight further suggests that enhancing the model’s awareness of these image tokens could be a beneficial direction.

\subsection{Attention Sinking on Textual Tokens}
\label{subsec:obs-4}
\textbf{Observation}:~
We conduct experiments with LLaVA-1.5 on the CHAIR benchmark, using 500 randomly selected images from the COCO validation set, as result shown in Figure~\ref{fig:onecol}. Visualizations of attention across layers reveal a significant attention sinking phenomenon in certain text tokens within the LVLM. Notably, these tokens tend to be tokens with low-semantic information, such as \texttt{<.>} and \texttt{<s>}.

\textbf{Insights}:~
Tokens with attention sinking in LVLM exhibit high attention scores and low semantic information, primarily concentrated in text tokens. This pattern suggests an intrinsic bias within LVLMs. However, excessive focus on low-semantic tokens may cause the model to rely heavily on linguistic priors and neglect the real visual information. Therefore, applying attention penalties to these sinking tokens during decoding could enhance the LVLM's perception of visual tokens.




\begin{table*}[htbp]
  \centering
      \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc}
    \toprule
     \multirow{2}[2]{*}{Methods} & \multicolumn{3}{c|}{LLaVA-1.5} & \multicolumn{3}{c|}{MiniGPT4} & \multicolumn{3}{c}{ mPLUG-Owl2} \\
          & CHAIR$_i\downarrow$ & CHAIR$_s\downarrow$ & TPS$\uparrow$   & CHAIR$_i\downarrow$ & CHAIR$_s\downarrow$ & TPS$\uparrow$   & CHAIR$_i\downarrow$ & CHAIR$_s\downarrow$ & TPS$\uparrow$ \\
    \midrule
     FastV & 8.53  & 26.76  & 33.21  & 16.72  & 41.32  & 38.29  & 11.40  & 38.49  & 24.6 \\
          SparseVLM & 8.44  & 26.11  & 32.47  & 16.38  & 40.93  & 37.81  & 11.35  & 38.99  & 23.73 \\
          Woodpecker & 6.72  & 19.79  & -     & 12.09  & 31.69  & -     & 8.99  & 25.05  & - \\
          LURE  & 6.67  & 19.75  & -     & 11.80  & 31.67  & -     & 7.78  & 22.53  & - \\
          Greedy & 7.22  & 22.20  & 31.25  & 12.17  & 31.47  & 36.64  & 8.94  & 24.42  & 20.36 \\
          Beam Search & 6.43  & 19.97  & 29.91  & 11.57  & 31.80  & 32.27  & 8.72  & 23.87  & 19.62 \\
          OPERA & 7.04  & 21.28  & 4.36  & 12.34  & 32.63  & 5.57  & 9.07  & 24.48 & 3.56 \\
         VCD   & 7.02  & 21.40  & 17.58  & 11.90  & 30.60  & 17.69  & 9.13  & 24.89  & 9.89 \\
          DoLa  & 6.44  & 20.23  & 23.61  & 11.62  & 30.58  & 25.01  & 8.88  & 24.67  & 14.74 \\
          SID   & 6.95  & 20.83  & 20.88  & 11.85  & 31.73  & 22.95  & 8.54  & 23.55  & 12.95 \\
          HALC  & 6.27  & 19.64  & 2.15  & 11.69  & 31.76  & 3.86  & 7.71  & 23.48  & 1.52 \\
          Ours  & \textbf{5.82 } & \textbf{18.51 } & 27.73  & 11.35  & 30.19  & 30.87  & 7.36  & 22.03  & 18.18 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
  \caption{Add caption}
  
\end{table*}%

\begin{table*}[htbp]
  \centering
      % \setlength{\tabcolsep}{2mm}{
          \resizebox{\textwidth}{!}{
  
    \begin{tabular}{c|ccc|ccc|ccc}
    \toprule
    \multirow{2}[2]{*}{Methods} & \multicolumn{3}{c|}{LLaVA-1.5} & \multicolumn{3}{c|}{MiniGPT-4} & \multicolumn{3}{c}{ mPLUG-Owl2} \\
          & Random & Popular & Adversarial & Random & Popular & Adversarial & Random & Popular & Adversarial \\
    \midrule
    Woodpecker & 59.73  & 58.53  & 58.07  & 53.84  & 51.70  & 51.27  & 58.10  & 53.07  & 55.42  \\
    LURE  & 60.08  & 58.63  & 58.34  & 53.91  & 52.37  & 51.38  & 58.28  & 53.15  & 55.65  \\
    Greedy & 58.75  & 57.42  & 56.64  & 53.71  & 51.68  & 51.92  & 57.40  & 53.43  & 55.43  \\
    Beam Search & 60.38  & 58.98  & 58.43  & 53.97  & 52.27  & 51.93  & 55.31  & 52.89  & 53.12  \\
    OPERA & 59.80  & 58.42  & 58.00  & 53.08  & 51.32  & 51.20  & 55.70  & 53.41  & 53.66  \\
    VCD   & 60.05  & 58.34  & 58.02  & 53.26  & 51.50  & 51.07  & \textbf{58.63 } & 54.87  & 56.13  \\
    DoLa  & 59.36  & 58.08  & 57.44  & 53.83  & 51.93  & 51.72  & 57.21  & 53.38  & 55.24  \\
    SID   & 61.63  & 59.62  & 58.83  & 53.86  & 51.98  & 51.77  & 55.82  & 53.46  & 56.07  \\
    HALC  & 60.46  & 59.33  & 58.50  & 53.93  & 52.06  & 51.80  & 56.29  & 53.38  & 55.84  \\
    Ours  & \textbf{62.13 } & \textbf{60.93 } & \textbf{59.20 } & \textbf{54.87 } & \textbf{52.93 } & \textbf{52.70 } & 58.27  & \textbf{55.28 } & \textbf{56.77 } \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
  \caption{Add caption}
\end{table*}%


\begin{table*}[htbp]
  \centering
      % \setlength{\tabcolsep}{1.8mm}{
          \resizebox{\textwidth}{!}{
    \begin{tabular}{cl|ccc|ccc}
    \toprule
    \multirow{2}[2]{*}{G.} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Settings}} & \multicolumn{3}{c|}{LLaVA-1.5} & \multicolumn{3}{c}{MiniGPT-4} \\
          &       & CHAIR$_i\downarrow$ & CHAIR$_s\downarrow$ &  TPS$\uparrow$  & CHAIR$_i\downarrow$ & CHAIR$_s\downarrow$ & TPS$\uparrow$ \\
    \midrule
    \multirow{2}[2]{*}{1} & w/o Whole Visual-Aware Token Selection & 6.43  & 19.75 & 25.54  & 11.63 & 30.51 & 27.55 \\
          & w/o Visual Perception Score P & 6.06  & 19.20  & 27.80  & 11.57 & 31.05 & 30.96 \\
    \midrule
    \multirow{2}[2]{*}{2} & w/o Whole SVCD & 6.91  & 21.42 & \textbf{30.68 } & 11.85 & 30.93 & \textbf{35.83} \\
          & w/o Mask-based Sparsification & 6.31  & 18.85 & 27.47  & 11.58 & 31.26 & 30.30  \\
    \midrule
    3     & w/o Sinking Attention Penalty & 6.32  & 19.39 & 27.96  & 11.52 & 31.04 & 30.92 \\
    \midrule
    4     & Our Full VASparse & \textbf{5.82} & \textbf{18.51} & 27.73  & \textbf{11.35} & \textbf{30.19} & 30.87 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
  \caption{Add caption}
  
\end{table*}%



\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{cccc}
    \toprule
          & \textbf{LLaVA-1.5} & \textbf{MiniGPT-4} & \textbf{mPLUG-Owl-2} \\
    \midrule
    Greedy & 36.3  & 46.7  & 42.3 \\
    OPERA & 34.2  & 45.9  & 41.7 \\
    VCD   & 34.6  & 46.0  & 41.9 \\
    HALC  & 33.9  & 45.8  & 41.7 \\
    Ours  & \textbf{33.5} & \textbf{45.2} & \textbf{41.1} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> sec/3_methods.tex <==
\section{Methods}
\label{sec:methods}

\subsection{Preliminaries}
We consider a general LVLM, symbolized as $\theta$, which is designed with an architecture that integrates a vision encoder, a vision-text interface, and a decoder of LLM.
Initially, the image $v$ undergoes processing through the vision encoder to produce a visual embedding, which is then modified by the vision-text interface (e.g., linear projector and Q-former~\cite{}) to align with the textual query $x$. The combined data serves as input to the text decoder, which autoregressively generates a textual output $y$ as:
\begin{equation}
\begin{aligned}
    y_t &\sim p_{\theta}(y_t | v, x, y_{<t}), \\
    p_{\theta}(y_t | v, x, y_{<t}) &\propto \exp\left( \operatorname{logit}_{\theta}(y_t | v, x, y_{<t}) \right),
\end{aligned}
\end{equation}
where, $y_t$ represents the $t$-th token of $y$, while $y_{<t}$ refers to the sequence of tokens generated prior to $t$-th step. The function $\operatorname{logit}_{\theta}$ is the logit distribution function.

The attention computation in each head of the LVLM decoder follows this protocol:
\begin{equation}
\operatorname{Attention}(Q, K) = \operatorname{Softmax}\left(\frac{Q K^\top}{\sqrt{d}}\right),
\end{equation}
where, $Q\in \mathbb{R}^{L\times D}$ and $K\in \mathbb{R}^{L\times D}$ are the query matrix and the key matrix, respectively, $D$ represents the dimension, and $L$ denotes the length of the sequence.
During decoding, $K$ and $V$ are derived from preceding decoding steps and stored in a key-value cache to avoid redundant computations. Consequently, the attention calculation for decoding the $t$-th token proceeds during decoding as follows:
\begin{equation}
\operatorname{Attention}(q_t, K_{\leq t}) = \operatorname{Softmax}\left(\frac{q_t K_{\leq t}^\top}{\sqrt{d}}\right)
\end{equation}
where $q_t$ is the query for the current decoding step, and $K_{\leq t}$ represents the keys up to and including step $t$.

When the generated token $y_t$ does not align with the input image $v$, VH occurs, which can distort the actual visual content.
Our primary goal is to reduce generated hallucinatory tokens to preserve the fidelity of the generated text and maintain efficient decoding speed.

\subsection{Problem Formulation}
Building on our empirical observations in Section~\ref{sec:obs}, we decompose the unified objective of achieving both trustworthiness and efficiency (\textit{i.e.}, reduced VH and accelerated decoding) for LVLMs into the following three sub-goals:


\textbf{Goal 1 (Token Sparsification)}:~
Given the sparsity of LVLMs (\textit{c.f.}, Section~\ref{subsec:obs-1}),
we define token sparsification through a binary sparse mask $M$, where each element $M_i \in \{0, 1\}$. An optimal sparsification minimizes $\sum_{i=1}^L M_i$ while maximizing the recall of attention scores, aiming for $q({M} \odot K)^\top$ to approximate the full attention score $qK^\top$ as closely as possible.

\textbf{Goal 2 (Vision-Aware Decoding)}:~
During decoding, some image tokens may hold lower attention scores but are crucial for decoding visually relevant instances. Ignoring these tokens can exacerbate visual hallucinations (\textit{c.f.}, Section~\ref{subsec:obs-2} and \ref{subsec:obs-3}). We assign each token a vision-aware saliency score $P_i$ to represent its importance for decoding visual instances. A higher $P_i$ indicates that the token should be more likely to be retained.

\textbf{Goal 3 (Penalizing Attention Sinking)}:~
Our observations (\textit{c.f.}, Section~\ref{subsec:obs-4}) indicate a pronounced attention sinking in LVLMs, where tokens receive disproportionately high attention scores despite low semantic information. Excessive focus on such tokens can blur visual information during decoding. Therefore, a targeted penalty should be applied to tokens exhibiting abnormally high attention scores. We define a penalty weight matrix $W = \operatorname{diag}\{w_1, \cdots, w_L\}$, where each $w_i$ serves as a penalty factor for anomalous attention scores.

The above objectives can be summarized as maintaining the original attention scores as much as possible while sparsifying the tokens and considering visual information during the decoding process. We innovatively unify these optimization goals into a constrained optimization problem. This optimization problem can be formalized as the error between the recalled attention scores and the original attention scores: 

\begin{Definition}
    \textbf{(Unified Objective)}:
    We define the joint objective of trustworthiness and efficiency in LVLMs as the solution to the following constrained optimization problem:
    \begin{equation}
    \begin{aligned}
    \min_{M} \quad \mathcal{E}(M) &= {\left\| qK^\top - q ({M} \odot K)^\top \right\|^2_{{W}}} - {\lambda P \cdot M} \\
    = \sum_{i=1}^L & {w_i} \left( \langle q, K_i \rangle - {M_i} \langle q, K_i \rangle \right)^2 - \lambda P_i \cdot M_i \\
    \text{s.t.} \quad M_i &\in \{0, 1\}, \quad \forall i = 1, 2, \dots, L; \\
    \sum_{i=1}^L M_i &= S,
    \end{aligned}
    \end{equation}
    where, $q \in \mathbb{R}^{1 \times D }$, $K_i \in K$ and $K_i \in \mathbb{R}^{1 \times D }$, $||\cdot||_W^2$ represents the weighted $L_2$ norm, \textit{e.g.}, $||v||_W^2 = v^\top W v$. $\langle \cdot,\cdot \rangle$ denotes the inner product, and $L$ is the sequence length, and $\lambda$ is a tradeoff parameter used to balance visual perception and attention recall.

\label{def:objective}
\end{Definition}

The objective~\ref{def:objective} inherently contains the following constraints:
(1) Sparsity Constraint: $\| M \| = S$, and $S$ denotes the number of non-zero elements in $M$, with $S < L$ and $M_i \in \{0, 1\}$; (2) Visual Saliency Constraint: $P = \{P_i\}_{i=1}^L$ represents the visual-aware scores; (3) Sinking Penalty: $W = \operatorname{diag}\{w_1, \cdots, w_L\}$ denotes the penalty weight for abnormal scores.
To solve this constrained optimization problem efficiently~\ref{def:objective}, we propose a novel visual-aware token selection strategy, sinking attention penalty to achieve efficient VH mitigation, and sparsification-based visual contrastive learning.


\subsection{Visual-Aware Token Selection}
\label{subsec:selection}
To solve the unified objective (\textit{Def}. \ref{def:objective}) and achieve efficient mitigation of visual hallucinations, we propose a visual-aware token selection strategy. Specifically, for each attention head, we rank tokens based on an aggregated score $\delta_i$ in descending order, and setting $M_i = 1$ for the top-$S$ tokens and $M_i = 0$ for the rest. The proposed aggregation score $\delta_i$ for each token $ M_i $ is defined as follows:
\begin{equation}
    \delta_i = w_i \left( \langle q, K_i \rangle \right)^2 + \lambda P_i,
\end{equation}
where, $\langle \cdot,\cdot \rangle$ denotes the inner product, the score $\delta_i$ combines both the weighted attention penalty $w_i$ and the visual saliency $P_i$, ensuring that the visually relevant tokens are retained while preserving computational efficiency.

\subsection{Sinking Attention Penalty} 

\subsection{Theoretical Analysis} 
\begin{Theorem}
\textbf{(Global Optimality)}: By employing the selection strategy defined in Section~\ref{subsec:selection}, we can obtain a globally optimal solution for the optimization problem defined in \textit{Def}.~\ref{def:objective}. Specifically, the sparse mask $M$ derived from this selection strategy satisfies:

\begin{equation}
    M^* = \arg \min_{M} \quad \mathcal {E}(M).
\end{equation}
\label{the:global}
\end{Theorem}

\textbf{Intuition:}~
A proof of the theorem~\ref{the:global} is provided in the appendix.
This theorem ensures that the proposed token selection strategy yields the minimal error $\mathcal{E}(M)$ for the objective, thus achieving global optimality in sparse token retention. 
This theoretical analysis further verifies the effectiveness of our approach in achieving both token sparsification and efficient visual perception.
